Leftover Lunch: Advantage-based Offline Reinforcement Learning for Language Models

Reinforcement Learning with Human Feedback (RLHF) is the most prominent method for Language Model (LM) alignment. However, RLHF is an unstable and data-hungry process that continually requires new high-quality LM-generated data for finetuning. We introduce Advantage-Leftover Lunch RL (A-LoL), a new class of offline policy gradient algorithms that enable RL training on any pre-existing data. By assuming the entire LM output sequence as a single action, A-LoL allows incorporating sequence-level classifiers or human-designed scoring functions as rewards. Subsequently, by using LM's value estimate, A-LoL only trains on positive advantage (leftover) data points, making it resilient to noise. Overall, A-LoL is an easy-to-implement, sample-efficient, and stable LM training recipe. We demonstrate the effectiveness of A-LoL and its variants with a set of four different language generation tasks. We compare against both online RL (PPO) and recent preference-based (DPO, PRO) and reward-based (GOLD) offline RL baselines. On the commonly-used RLHF benchmark, Helpful and Harmless Assistant (HHA), LMs trained with A-LoL methods achieve the highest diversity while also being rated more safe and helpful than the baselines according to humans. Additionally, in the remaining three tasks, A-LoL could optimize multiple distinct reward functions even when using noisy or suboptimal training data. We also release our experimental code. https://github.com/abaheti95/LoL-RL

==> tables/poster_hha_table.tex <==
\begin{table*}[t]
\caption{HHA aggregate test reward and diversity evaluation of NLL, PPO, and other offline RL methods averaged across three random seeds. For comparison, we also report the performance of Test responses and reference policy ($\pi_{\text{ref}}$) in the first three rows, along with another external PPO model* in the last row. Overall, the best {\alol} methods achieve comparable rewards to DPO, while approaching the distribution of Test \textit{good} responses in terms of length and diversity. Oddly, DPO and DPO (ref. free) tend to generate \underline{longer and less diverse} responses while PPO generates the shortest.} 
% \faeze{test good test bad rows are not super clear as they are under Algorithm columns. Maybe explain it in the caption?}
\label{tab:main_result_poster}
\centering
\small
% \resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|c|cc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Algorithm}}  & \multirow{2}{*}{\parbox{1cm}{\centering Avg. Reward}} & \multirow{2}{*}{\parbox{1cm}{\centering Avg. Length}} & \multirow{2}{*}{\parbox{2.3cm}{\centering Diversity: \\ Avg Distinct-1,2,3}} \\ 
&&&\\
\cmidrule(lr){1-1}
\multicolumn{1}{c|}{\#instances} & (8207) & & \\
\midrule
% Test \textit{good} responses & $50.3$ & $46.7$ & $.099$/$.471$/$.773$ \\
% Test \textit{bad} responses & $45.4$ & $45.3$ & $.099$/$.468$/$.771$ \\
$\pi_{\text{ref}}$ \hfill (LLaMA-7B) & $44.7$ & $51.1$ & $.067$/$.246$/$.404$ \\
\midrule
+ SFT or NLL & $51.9_{\pm0.5 }$ & $43.3_{\pm3.5 }$ & $.084$/$.336$/$.552$ \\
\midrule
\multicolumn{4}{l}{\textit{Preference-based offline RL}}\\
\midrule
+ PRO & $54.1_{\pm0.6 }$ & $43.4_{\pm2.5 }$ & $.084$/$.339$/$.560$ \\
+ DPO (ref. free) & $52.3_{\pm1.4 }$ & \underline{$90.5_{\pm1.1 }$} & \underline{$.049$/$.226$/$.432$} \\
+ DPO & $\mathbf{58.6_{\pm0.8 }}$ & \underline{$66.7_{\pm5.9 }$} & \underline{$.065$/$.288$/$.503$} \\
\midrule
\multicolumn{4}{l}{\textit{Reward-based offline RL}}\\
\midrule
+ wBC & $54.8_{\pm0.4 }$ & $42.7_{\pm1.1 }$ & $.091$/$.380$/$.622$ \\
+ R GOLD & $54.5_{\pm0.3 }$ & $44.2_{\pm3.1 }$ & $.086$/$.355$/$.584$ \\
+ {\rlol} & $55.1_{\pm0.6 }$ & $38.6_{\pm2.4 }$ & $.095$/$.394$/$.640$ \\
\midrule
\multicolumn{4}{l}{\textit{Advantage-based offline RL}}\\
\midrule
+ {\alol} (ref. free) & $56.4_{\pm0.6 }$ & $40.7_{\pm1.7 }$ & $.095$/$.400$/$.651$ \\
+ {\alol} & $57.3_{\pm0.3 }$ & $42.3_{\pm1.9 }$ & $.094$/$.403$/$.657$ \\
+ {\alol} seq. & $57.6_{\pm0.5 }$ & $40.1_{\pm2.4 }$ & $.105$/$\mathbf{.464}$/$\mathbf{.727}$ \\
+ {\alol} KL & $\mathbf{57.9_{\pm0.3 }}$ & $44.0_{\pm1.7 }$ & $.090$/$.387$/$.639$ \\
\midrule
\multicolumn{4}{l}{\textit{Online RL}}\\
\midrule
% Older result with 3 epochs
% + PPO & $63.3$ & $39.9$ & $48.0$ & $43.5$ & $48.4_{\pm2.1 }$ & $18.7_{\pm1.0 }$ & $\mathbf{.114}$/$.355$/$.512$ \\
+ PPO & $48.0_{\pm0.2 }$ & $16.9_{\pm0.6 }$ & $\mathbf{.123}$/$.381$/$.546$ \\
% PPO* (pythia 6B) & $37.1$ & $13.3$ & $.094$/$.301$/$.447$ \\
% PPO (GPT neo X 20B) & $42.0$ & TBD \\
\bottomrule
\end{tabular}
% } %(end resizebox)

\end{table*}

==> tables/poster_table.tex <==
\begin{table}[t]
\centering
\caption{Properties of existing offline and online RL algorithms\protect\footnotemark compared to {\alol} and its variants.}
%  We do not report the test results if finetuning the reference policy further doesn't increase the validation success measure.
\label{tab:comparison_poster}

\scriptsize
% \begin{wraptable}{r}{7cm}
% \resizebox{7cm}{!}{
\begin{tabular}{l|ccccc}
\toprule
\multirow{2}{*}{Algorithm} & \multirow{2}{*}{\parbox{2cm}{\centering Needs Human Preference Data?}} & \multirow{2}{*}{\parbox{1.3cm}{\centering Action \\ Representation}} & \multirow{2}{*}{\parbox{1.2cm}{\centering Reference LM}} & \multirow{2}{*}{Rewards} & \multirow{2}{*}{Advantage} \\ 
\\
\midrule
NLL (negative log-likelihood) & No & N/A & \xmark & \xmark & \xmark \\ 
\midrule
\multicolumn{5}{l}{\textit{Preference-based offline RL}}\\
\midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.2cm}{\centering Preference-based Offline RL}}} &&&\\
DPO \hfill \cite{rafailov2023direct} & Yes & Sequence & \cmark & \xmark & \xmark \\ 
DPO (ref. free) \hfill \cite{rafailov2023direct} & Yes & Sequence & \xmark & \xmark & \xmark \\ 
PRO \hfill \cite{song2023pro} & Yes & Sequence & \cmark & \cmark & \xmark \\ 
\midrule
\multicolumn{5}{l}{\textit{Reward-based offline RL}}\\
\midrule 
wBC \hfill \cite{NEURIPS2020_588cb956} & No & Tok./Seq. & \xmark & \cmark & \xmark \\ 
GOLD \hfill \cite{pang2021text} & No & Token & \xmark & \cmark & \xmark \\ 
\midrule 
\multicolumn{5}{l}{\textit{Advantage-based offline RL}}\\
\midrule 
{\alol} \hfill (ours) & No & Sequence & \cmark & \cmark & \cmark \\ 
~$\triangleright$ {\rlol} \hfill (variant) & No & Sequence & \cmark & \cmark & \xmark \\ 
~$\triangleright$ {\alol} (ref. free) \hfill (variant) & No & Sequence & \xmark & \cmark & \cmark \\ 
~$\triangleright$ {\alol} seq. \hfill (variant) & No & Sequence & \cmark & \cmark & \cmark \\ 
~$\triangleright$ {\alol} KL \hfill (variant) & No & Sequence & \cmark & \cmark & \cmark \\ 
\midrule
\multicolumn{5}{l}{\textit{Online Reinforcement Learning with Human Feedback}}\\
\midrule 
PPO \hfill \cite{schulman2017proximal} & No & Tok./Seq. & \cmark & \cmark & \cmark \\ 
\bottomrule
\end{tabular}
% } %(end resizebox)
% \captionsetup{font=scriptsize}

\end{table}
